Optimal randomized incremental construction for guaranteed logarithmic planar point location

Given a planar map of $n$ segments in which we wish to efficiently locate points, we present the first randomized incremental construction of the well-known trapezoidal-map search-structure that only requires expected $O(n \log n)$ preprocessing time while deterministically guaranteeing worst-case linear storage space and worst-case logarithmic query time. This settles a long standing open problem; the best previously known construction time of such a structure, which is based on a directed acyclic graph, so-called the history DAG, and with the above worst-case space and query-time guarantees, was expected $O(n \log^2 n)$. The result is based on a deeper understanding of the structure of the history DAG, its depth in relation to the length of its longest search path, as well as its correspondence to the trapezoidal search tree. Our results immediately extend to planar maps induced by finite collections of pairwise interior disjoint well-behaved curves.

==> dag_size.tex <==
\label{appendix_dag_size}
In order to derive data structures with guaranteed
worst-case size and query time bounds,
while using a randomized incremental
construction (see Theorems~\ref{thrm:gnrl_preproc_time} and~\ref{thrm:new}),
expected resource bounds are insufficient.
We need to provide stronger bounds on the
so-called tail estimates for the size of these resources:
bounding the probability that a resource bound is above a certain threshold.
A tail estimate for the query time is analyzed in \cite[Chapter~6]{CG-alg-app}.
For completeness we provide here a tail-estimate analysis
for the size of the structure; see also~\cite{Kleinbort_master}.

\begin{lemma}
\label{appendix:sizeprob}
Let $S$ be a set of $n$ non-crossing $x$-monotone curves,
and let $\rho \geq 1$ be a parameter.
The probability that \calS
is more than $15\rho n$ is at most
$\frac{1}{\rho}$.
\end{lemma}

\begin{proof}
Let \calC be a non-negative random variable representing
the number of DAG nodes, i.e., the size \calS of the
search structure.
\calC is composed of the number of leaves in the final search structure
and the sum of inner nodes created in all iterations.
The number of leaves equals to $|\calTS|$, the number of trapezoids in
the final trapezoidal map. Hence, it is at most~$3n + 1$.
%As shown in~\cite{CG-alg-app} when proving the expected size,
Let~$k_i$ denote the number of trapezoids created by the
insertion of the $i$th curve.
Let $\calASi$ denote the arrangement of the first $i$ curves,
and \calTSi denote the matching trapezoidal map for this arrangement.
%Clearly, the number of inner nodes created in iteration $i$
%equals to $k_i - 1$.
%
The number of inner nodes created in iteration $i$
is equal to the number of trapezoids that are split by
the interior (not endpoints) of the inserted curve $cv_i$
plus the number of
endpoints of $cv_i$ that do not exist in the
current structure \calTSiminus.
%
In fact, we can count the number of vertical walls
that are blocked by the $cv_i$ (which is equal
to the number of trapezoids that are split by
the interior of $cv_i$ minus $1$), since the
trapezoid lying on the left side of the blocked wall
is new.
If the left endpoint of~$cv_i$ is inserted to the structure
(an inner node for this endpoint is added)
then a new trapezoid to its left is added.
Similarly, if the right endpoint of $cv_i$
is inserted to the structure
then a new trapezoid to its right is added.
%
Therefore, the number of inner nodes created in iteration
$i$ is exactly the number of new trapezoids
created in the same iteration minus 1, i.e., $k_i - 1$.

The expected number of DAG nodes, $\mathbb{E}[\calC]$,
can be bounded as follows:
\begin{dmath*}
\mathbb{E}[\calC] = \mathbb{E}[|\calTS| + \sum\limits_{i=1}^n {(k_i-1)}]
= \mathbb{E}[|\calTS|] + \mathbb{E}[\sum\limits_{i=1}^n {(k_i-1)}]
= \mathbb{E}[|\calTS|] + \mathbb{E}[\sum\limits_{i=1}^n k_i] - n
\leq (3n+1) + \mathbb{E}[\sum\limits_{i=1}^n k_i] - n
= 2n + 1 + \mathbb{E}[\sum\limits_{i=1}^n k_i]
\end{dmath*}.
Using linearity of expectation we get:
$$\mathbb{E}[\calC] \leq 2n + 1 + \sum\limits_{i=1}^n \mathbb{E}[k_i].$$
The expected number of new trapezoids created in the $i$th
iteration can be bounded using the following backwards analysis.
Each trapezoid is defined by at most four curves and by
removing one of these curves the trapezoid is destroyed.
If $cv_i$, the $i$th inserted curve, is removed from
\calTSi, the probability that a given
trapezoid $\Delta$ is destroyed is at most $4/i$.
Since $|\calTSi|$ is the number of trapezoids in the
trapezoidal map for the first $i$ inserted curves,
the expected number of trapezoids that are destroyed if
$cv_i$ is removed from \calTSi is at
most~$|\calTSi|\cdot 4/i$,
which is the expected number of new
trapezoids created in the $i$th
iteration.
In addition, as we already mentioned, the number of trapezoids
in a trapezoidal map of $i$ curves in general position is
at most~$3i + 1$.
Therefore,~$\mathbb{E}[k_i]$ can be bounded as follows:
\begin{dmath*}
{\mathbb{E}[k_i]\leq\frac{4\cdot|\calTSi|}{i}}
\leq {\frac{4(3i+1)}{i} = 12 + \frac{4}{i}}
\end{dmath*}.
Putting it all together:
\begin{dmath*}[compact]
\mathbb{E}[\calC] \leq 2n + 1 + \sum\limits_{i=1}^n {(12+\frac{4}{i})}
= 14n + 1 + 4\sum\limits_{i=1}^n \frac{1}{i}
= 14n + 1 + 4H_n
\end{dmath*},
where $H_n$ is the $n$-th harmonic number and $\ln n < H_n < \ln n + 1$, and therefore:
$$\mathbb{E}[\calC] < 14n + 4\ln n + 2 < 15n \text{, for } n\geq 12 .$$

Since \calC is a non-negative random variable we can use Markov's inequality,
according to which for any $\alpha > 0$ we have:
$$ \Pr[\calC \geq \alpha] \leq \frac{\mathbb{E}[\calC]}{\alpha} .$$
Now, we choose $\alpha = 15\rho n$ and substitute
$$ \Pr[\calC \geq 15\rho n] \leq \frac{\mathbb{E}[\calC]}{15\rho n}
= \frac{15n}{15\rho n} = \frac{1}{\rho} .$$
\myqed
\end{proof} 

==> expected_tree_size.tex <==

The following lemma bounds the expected size of \TrpSrchTree to be $O(n \log n)$. 
\begin{lemma}
\label{lemma:tree_size}
Let $S$ be a set of $n$
pairwise interior disjoint $x$-monotone curves
inducing a planar subdivision.
The expected number of leaves
in the trapezoidal search tree \TrpSrchTree,
which is constructed as the DAG but without merges,
is $O(n\log{n})$.
\end{lemma}

\begin{proof}
We would like to bound the expected number
of leaves in~\TrpSrchTree, namely,
the expected number
of trapezoids in the decomposition without merges.
We can symbolically shorten every curve at its two endpoints
by an arbitrarily small value, namely $\epsilon$.
In other words, if a curve $cv$ %$cv_i$ 
has an $x$-range $(a,b)$,
then the shortened curve will have an $x$-range $(a+\epsilon, b-\epsilon)$.
The curves of the updated subdivision are now completely disjoint.
In addition, this operation gave rise to new artificial trapezoids.
Clearly, for any point $p$ in such an artificial trapezoid,
we can decrease the value of $\epsilon$ such that $p$ will not be
covered by this trapezoid.
Now we would like to bound the number of trapezoids in the set
of shortened curves.
It is clearly bounded by the number of vertical edges + 1.
First, consider the vertical line~$W$ through one endpoint of a curve $cv$.
$W$ is intersected by $m$ curves.
Suppose that $cv$ is the $i$th inserted curve among these $m$ curves.
The $i-1$ already inserted curves partition $W$ into $i$ intervals.
However, we are only interested in the interval $I$ containing the
endpoint of $cv$, as it will
appear in the final structure.
Curves inserted after $cv$ may split $I$.
The expected number of intersections in $I$
(including the endpoint of $cv$) is $O((m-i)/i)$.
The probability that $cv$ will be inserted $i$th is $\frac{1}{m}$.
Summing up over all possible insertion orders we get that the expected number
of intersection in $I$ is $\sum\limits_{i=1}^{m} \frac{1}{m}\cdot\frac{(m-i)}{i} = O(\log{m})$.
However, since $m \leq n$, 
this number can be bounded $O(\log{n})$.
There are $O(n)$ vertical walls, giving a total of expected $O(n\log{n})$ intersections.
Thus, the expected number of vertical edges is $O(n\log{n})$ as well,
and, clearly, this is also the expected number of leaves in the tree.


\ignore{
First, consider the vertical line~$W$ through one endpoint of the %focus on a vertical wall $W$ induced by one endpoint of the
$i$th inserted curve.
$W$ is intersected by $n$ curves, in the worst case.
The $i-1$ already inserted curves partition $W$ into $i$ intervals.
However, we are only interested in the interval $I$ containing the
endpoint of the $i$th curve, as it will
appear in the final structure.
Curves inserted after the $i$th curve may split $I$.
The expected number of intersections in $I$
(including the endpoint of the $i$th curve) is $O((n-i)/i)$.
Summing up over all vertical walls gives a total of expected $O(n\log{n})$ intersections.
Thus, the expected number of vertical edges is $O(n\log{n})$ as well,
and, clearly, this is also the expected number of leaves in the tree.}
\qed
\end{proof}

